Numerical evaluation of stress intensity factors and T-stress for interfacial cracks and cracks terminating at the interface without asymptotic enrichment

In this paper, we extend the recently proposed extended scaled boundary finite element method (xSBFEM)~\cite{natarajansong2013} to study fracture parameters of interfacial cracks and cracks terminating at the interface. The approach is also applied to crack growth along the interface and crack deflecting into the material within the context of linear elastic fracture mechanics. Apart from the stress intensity factors, the T-stress can be computed directly from the definitions, without any requirement of path independent integrals. The method aims at improving the capability of the extended finite element method in treating crack tip singularities of cracks at interfaces. An optimum size of the scaled boundary region is presented for multimaterial junctions. The proposed method: (1) does not require special numerical integration technique; (2) does not require a priori knowledge of the asymptotic fields and (3) the stiffness of the region containing the crack tip is computed directly. The robustness of the proposed approach is demonstrated with a few examples in the context of linear elastic fracture mechanics. A discussion on the crack growth along the interface and crack deflecting into the material is also presented.

==> EnrichmentFunction.tex <==
\subsection{Summary of enrichment functions} In this section, we present the different enrichment functions proposed in the literature to study crack tip fields in isotropic and orthotropic medium. We also discuss techniques adopted to compute the enrichment functions when a closed form is not available or is very complex.

\paragraph*{Isotropic material} For isotropic materials, the near-tip function, $\Xi_{\alpha}$ in \Eref{eqn:uS2} is denoted by $\{B_\alpha\}_{1 \leq \alpha \leq 4}$ and is given by:
\begin{equation}
\{ B_\alpha\}_{1 \leq \alpha \leq 4} (r,\theta)= \sqrt{r} \left\{
\sin \frac{\theta}{2},
\cos \frac{\theta}{2}, \sin \theta
\sin \frac{\theta}{2}, \sin \theta
\cos \frac{\theta}{2} \right\}.
\label{eq:asymptotic}
\end{equation}
where $(r,\theta)$ are the crack tip polar coordinates.


\paragraph*{Orthotropic material}
For the case of orthotropic materials, the asymptotic functions given by \Eref{eq:asymptotic} has to be modified because the material property is a function of material orientation. Asadpoure and Mohammadi~\cite{asadpouremohammadi2007} proposed special near-tip functions for orthotropic materials as
\begin{equation}
\{B_\alpha\}_{1 \leq \alpha \leq 4} (r,\theta)= \sqrt{r} \left\{
\cos \frac{\theta_1}{2} \sqrt{g_1(\theta)},
\cos \frac{\theta_2}{2} \sqrt{g_2(\theta)},
\sin \frac{\theta_1}{2} \sqrt{g_1(\theta)},
\sin \frac{\theta_2}{2} \sqrt{g_2(\theta)} \right\}.
\label{eq:orthoasymptotic}
\end{equation}
where $(r,\theta)$ are the crack tip polar coordinates. The functions $g_i (i=1,2)$ and $\theta_i (i=1,2)$ are given by
\begin{eqnarray}
g_j(\theta) = \left( \cos^2 \theta + \frac{\sin ^2 \theta}{e_j^2} \right), \hspace{0.5cm} j=1,2 \nonumber \\
\theta_j = \arctan \left( \frac{\tan \theta}{e_j} \right), \hspace{0.5cm} j=1,2
\end{eqnarray}
where $e_j (j=1,2)$ are related to material constants, which depend on the orientation of the material~\cite{asadpouremohammadi2007}. These new enrichment functions for orthotropic material were applied to uni-directional fibre reinforced composite and the results from the XFEM were found to be in very good agreement with the experimental results~\cite{cahillnatarajan2014}.  The PUM has been extended to study matrix failures and debonding in thin fibre composites~\cite{simone2004,radtkesimone2011}.

\paragraph*{Anisotropic material} Hattori \textit{et al.,}~\cite{hattorirojas-diaz2012} derived the following new set of anistropic crack tip-enrichment functions based on Stroh's formalism. The set of functions that span the asymptotic fields ahead of crack in an anisotropic material are:
\begin{equation}
\mathbf{F}(r,\theta) = \sqrt{r} \left( \Re \left[ \frac{ \mathbf{B}^{-1} \mathbf{A}_1 \boldsymbol{\beta}}{\mathbf{B}^{-1} \mathbf{A}_2 \boldsymbol{\beta}} \right] \right)
\end{equation}
where $\mathbf{A}_1$ and $\mathbf{A}_2$ correspond to the first and second row of a matrix $\mathbf{A}$. The matrices $\mathbf{A}$ and $\mathbf{B}$ depend on the material property and
\begin{equation}
\beta_i = \sqrt{ \cos \theta + \mu_i \sin \theta}
\end{equation}
where $\mu_i$ are the eigen values. For detailed derivation and discussion, interested readers are referred to~\cite{hattorirojas-diaz2012}.

\paragraph*{Bimaterial interface crack}
Based on the near tip asymptotic displacement fields, Sukumar \textit{et al.,}~\cite{sukumarhuang2004} derived the following set of enrichment functions that span the asymptotic fields for an crack aligned to the bimaterial interface:
\begin{equation}
\begin{split}
\{B_\alpha\}_{1 \leq \alpha \leq 12} (r,\theta) = \left\{ \sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{-\epsilon\theta}\sin{\frac{\theta}{2}}, 
\sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\sin{\frac{\theta}{2}}\sin{\theta},  \sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{-\epsilon\theta}\cos{\frac{\theta}{2}}, \right. \\
\left. \sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\cos{\frac{\theta}{2}}\sin{\theta}, \sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\sin{\frac{\theta}{2}},  \sqrt{r}\sin(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\sin{\frac{\theta}{2}}\sin{\theta}, \right. \\
\left.  \sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\cos{\frac{\theta}{2}}, \sqrt{r}\sin(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\cos{\frac{\theta}{2}}\sin{\theta}, \sqrt{r}\sin(\epsilon \mathrm{log}r)\mathrm{e}^{-\epsilon\theta}\sin{\frac{\theta}{2}},  \sqrt{r}\cos(\epsilon \mathrm{log}r)\mathrm{e}^{-\epsilon\theta}\sin{\frac{\theta}{2}}\sin{\theta}, \right. \\
\left.  \sqrt{r}\sin(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\sin{\frac{\theta}{2}}, \sqrt{r}\sin(\epsilon \mathrm{log}r)\mathrm{e}^{\epsilon\theta}\sin{\frac{\theta}{2}}\sin{\theta}. \right\}
\end{split}
\label{eqn:bimatincrack}
\end{equation}
where $\epsilon$ is the bimaterial constant, also referred to as the oscillatory index, given by:
\begin{equation}
\epsilon = \frac{1}{2\pi} \mathrm{log} \left( \frac{1 - \beta}{1+\beta} \right)
\label{eqn:osciindex}
\end{equation}
where $\beta$ is the second Dundur's parameter
\begin{equation}
\beta = \frac{\mu_1(\kappa_2-1) + \mu_2(\kappa_1-1)}{\mu_1(\kappa_2+1) + \mu_2(\kappa_1+1)}
\end{equation}
and,
\begin{equation}
\kappa_i = \left\{ \begin{array}{cr} (3-\nu_i)/(1+\nu_i) & \textup{plane stress} \\ 3 -4\nu_i & \textup{plane strain} \end{array} \right.
\end{equation}
where $\mu_i, \nu_i$ and $\kappa_i, (i=1,2)$ are the shear modulus, Poisson's ratio and the Kolosov coefficient, respectively. If the bimaterial constant $\epsilon=0$, the span of the enrichment functions given by \Eref{eqn:bimatincrack} degenerates to the isotropic asymptotic fields given by \Eref{eq:asymptotic}. Esna Ashari and Mohammadi~\cite{asharimohammadi2011} derived interlaminar crack tip enrichment functions from analytical asymptotic displacement fields around a traction free interfacial crack. The set of functions that span the asymptotic fields for a bimaterial interface crack in an orthotropic medium are:
\begin{equation}
\{B_\alpha\}_{1 \leq \alpha \leq 8} (r,\theta) = \sqrt{r_z} e^{\mu \epsilon \theta_z} S_j \left( \epsilon \mathrm{log} r_z - \mu \frac{\theta_z}{2} \right)
\end{equation}
where 
\begin{equation}
S_j = \left\{ \begin{array}{cc} \cos() & j=1,3,5,7 \\ \sin() & j=2,4,6,8 \end{array} \right., \hspace{0.2cm} z = \left\{ \begin{array}{cc} \ell & j = 1-4 \\ s & j =5-8 \end{array} \right. , \hspace{0.2cm} \mu = \left\{ \begin{array}{cc} 1 & j=3,4,7,8 \\ -1 & j=1,2,5,6 \end{array} \right.
\end{equation}
where $r_z, \theta_z (z=\ell,s)$ are related to polar coordinate system $(r,\theta)$ as
\begin{equation*}
r_z = r\sqrt{ \cos^2 \theta + Z_z^2 \sin^2 \theta}, \hspace{0.2cm} \theta_z = \textup{atan}(Z_z \tan \theta)
\end{equation*}
where $Z_z$ is a function of material properties~\cite{asharimohammadi2011}.

\paragraph*{Crack terminating at a bimaterial interface} Bouhala \textit{et al.,}~\cite{bouhalashao2013} derived new set of enrichment functions for a crack terminating at a bimaterial interface by considering plane elasticity solution based on Airy functions. The stress intensity factors were calculated based on the body force method. For a crack perpendicular to the bi-material interface, the enrichment functions are:
\begin{equation}
\{B_\alpha\}_{1 \leq \alpha \leq 4} (r,\theta) = r^\lambda \left\{ \cos(\lambda+1)\theta, \sin(\lambda+1)\theta, \cos(\lambda-1)\theta, \sin(\lambda-1)\theta \right\}
\end{equation}
where $\lambda$ indicates the strength of singularity. In the case of an oblique crack, the exponent $\lambda$ is real and double, denoted by $\lambda_1$ and $\lambda_2$. For an oblique crack, the enrichment functions are given by:
\begin{equation}
\begin{split}
\{B_\alpha\}_{1 \leq \alpha \leq 8} (r,\theta) = \left[ r^{\lambda_1} \left\{ \cos(\lambda_1+1)\theta, \sin(\lambda_1+1)\theta, \cos(\lambda_1-1)\theta, \sin(\lambda_1-1)\theta \right\}, \right.  \\
\left. r^{\lambda_2} \left\{ \cos(\lambda_2+1)\theta, \sin(\lambda_2+1)\theta, \cos(\lambda_2-1)\theta, \sin(\lambda_2-1)\theta \right\} \right]
\end{split}
\end{equation}

\paragraph*{Numerically determined enrichment functions} As seen from above, different set of enrichment functions are required to represent the asymptotic fields ahead of the crack tip. This depends on the material property. These functions for general heterogenous materials are very complex. To circumvent this problem, these functions can be computed by adopting a numerical procedure. A global-local approach was adopted by Duarte and Kim~\cite{duartekim2008} to build numerical enrichment functions. In their approach, first the global problem is solved over a coarse mesh and the solution of which is applied as the boundary conditions for a local problem, specifically designed to capture the local features. The solution of the local problem is then used as enrichment functions. Waisman and Belytschko~\cite{waismanbelytschko2008} find enrichment functions that are unknown in advance by using parametric enrichment functions that depend on unknown parameters. By minimizing an a-posteriori error estimate, these unknown parameters are estimated. Li \textit{et al.,}~\cite{lizhang2001} and Papadakis and Babu\v{s}ka~\cite{papadakisbabuvska1995} estimated the singular strain fields in anisotropic wedges numerically. This was latter employed within the context of the XFEM by Menk and Bordas~\cite{menkbordas2010}. Although computationally expensive, this method gives a systematic procedure to compute the enrichment functions when their analytical form is not known a priori. Mousavi \textit{et al.,}~\cite{mousavigrinspun2011,mousavigrinspun2011a} based on the work of Kaufmann \textit{et al.,}~\cite{kaufmannmartin2009} computed numerically the enrichment functions, by solving a Laplace equation over the domain enriched for any cracks. In~\cite{mousavigrinspun2011}, the local problem is solved separately, unlike the work of Duarte and Kim~\cite{duartekim2008}, where the global-local problems are coupled. The approach can readily be applied to arbitrary and branched cracks, but the accuracy of which is depends on the discretization of the local problem. Morevoer, it is limited to the case of cracks in homogeneous materials. Zhu~\cite{zhu2012} presented a mathematical derivation of the enrichment functions by coupling the level set method with characteristic functions as well as the domain decomposition and reproduction technique. 

==> OrderOfSing.tex <==
\subsection{Order of singularities in multimaterial wedges and interface cracks}


%--- figures depiciting the problems... L shape, iso domain with crack, bimaterial interface crack and crack terminating at the interface....
\begin{figure}[htpb]
\centering
\subfigure[L-shaped structure]{\scalebox{0.7}{\input{./Figures/lshape.pstex_t}}}
\subfigure[Crack in an isotropic medium]{\scalebox{0.7}{\input{./Figures/isocrk.pstex_t}}}
\subfigure[Bi-material interface crack]{\scalebox{0.7}{\input{./Figures/bimatcrk.pstex_t}}}
\subfigure[Crack terminating at an interface]{\scalebox{0.7}{\input{./Figures/trimat.pstex_t}}}
\caption{Estimation of the order of singularity: problem description}
\label{fig:probdescription}
\end{figure}

\paragraph{L-shaped domain}


% convergence of the relative error in displacement .....
\begin{figure}
\centering
\newlength\figureheight 
\newlength\figurewidth 
\setlength\figureheight{8cm} 
\setlength\figurewidth{10cm}
\subfigure[$\lambda_1$]{\input{./Figures/lshape_lam1.tikz}}
\subfigure[$\lambda_2$]{\input{./Figures/lshape_lam2.tikz}}
\caption{L-shaped problem: Convergence of order of singularity}
\label{fig:lshpResults}
\end{figure}

\paragraph{Crack in an isotropic medium}


% convergence of the relative error in displacement .....
\begin{figure}
\centering
%\newlength\figureheight 
%\newlength\figurewidth 
\setlength\figureheight{8cm} 
\setlength\figurewidth{10cm}
\subfigure[Relative error in displacement, $u_x$]{\input{./Figures/isocrkux.tikz}}
\subfigure[Relative error in displacement, $u_y$]{\input{./Figures/isocrkuy.tikz}}
\caption{Crack in an isotropic medium: Convergence in the relative error in the displacement.}
\label{fig:lshpResults}
\end{figure}

\paragraph{Bimaterial interface crack}

\paragraph{Crack terminating at a bimaterial interface}

==> SBFEM_crack.tex <==
%% LyX 2.0.6 created this file.  For more info, see http://www.lyx.org/.
%% Do not edit unless you really know what you are doing.
%\documentclass[english]{article}
%\usepackage[T1]{fontenc}
%\usepackage[latin9]{inputenc}
%\usepackage{amsmath}
%\usepackage{babel}
\begin{document}
Using Eq.~(21), the polar coordinates $r$ and $\theta$ are expressed
in the scaled boundary coordinates $\xi$ and $\eta$ as 
\begin{align}
r(\xi,\eta) & =\xi r_{\eta}(\eta)=\xi\sqrt{x_{\eta}^{2}(\eta)+y_{\eta}^{2}(\eta)}\label{eq-polar-r}\\
\theta(\eta) & =\arctan\dfrac{y_{\eta}(\eta)}{x_{\eta}(\eta)}\label{eq-polar-theta}
\end{align}
where $r_{\eta}(\eta)$ is the radial coordinate on the boundary.
The angle $\theta(\eta)$ is a single-valued function in its principal
value ($-\pi<\theta\leq\pi$). The element number and the local coordinate
$\eta$ can be regarded as a discrete representation of the angle
$\theta$. 

An attractive feature of the scaled boundary finite element method
is that no a prior knowledge of the asymptotic solution is require
to accurately handle the stress singularity at a crack tip. When the
scaling centre is placed at the crack tip, the solution for the stress
field in Eq.~(41) is expressed, by using Eq.~(\ref{eq-polar-r}),
as

\begin{equation}
\boldsymbol{\sigma}(r,\eta)=\sum_{i=1}^{n}c_{i}r^{-(\lambda_{i}+1)}\left(r_{\eta}^{\lambda_{i}+1}(\eta)\boldsymbol{\psi}_{\sigma i}(\eta)\right)\label{eq-stress-bd-slu}
\end{equation}
where $\boldsymbol{\psi}_{\sigma i}(\eta)$  is the $i-$th stress
mode, i.e. the $i-$th column of the matrix $\boldsymbol{\Psi}_{\sigma}(\eta)$.
Like the well-known William expansion (Reference? ), Eq.~(\ref{eq-stress-bd-slu})
is a power series of the radial coordinate $r$. The radial variation
of each term of the series is expressed analytically by the power
function $r^{-(\lambda_{i}+1)}$. At discrete points along the boundary,
the angular coordinates (Eq.~(\ref{eq-polar-theta})) are arranged
as a vector $\boldsymbol{\theta}(\eta)$ and the stress modes $\boldsymbol{\psi}_{\sigma i}(\eta)$
are computed. $\boldsymbol{\psi}_{\sigma i}(\eta)$ and $\boldsymbol{\theta}(\eta)$
form a parametric equation of the angular variation of stresses. 

The singular stress and T-stress terms can be easily identified by
the value of the exponent $-(\lambda_{i}+1)$. When the real part
of the exponent $-(\lambda_{i}+1)$ of a term is negative, the stresses
of this term at the crack tip, i.e. $\xi=0$, tend to infinity. When
the exponent $-(\lambda_{i}+1)$ of a term is equal to $0$, the stresses
of this term are constant and contribute to the $T-$stress. 

In the case of a crack in a homogeneous material, as shown in Section~5.1,
two singular terms exist in the solution and the order of singularity
($\lambda_{i}+1$) converges to $0.5$. Denoting the singular stress
modes as $I$ and $II$, the singular stresses (superscript $\mathrm{s}$
for singular stresses) are expressed as
\begin{equation}
\boldsymbol{\sigma}^{\mathrm{s}}(r,\eta)=\sum_{i=I,II}c_{i}r^{-(\lambda_{i}+1)}\left(r_{\eta}^{\lambda_{i}+1}(\eta)\boldsymbol{\psi}_{\sigma i}(\eta)\right)\label{eq:singularStress}
\end{equation}
Note that the singular stress terms are separated from other terms
and the stress singularity is represented analytically. This allows
the evaluation of the stress intensity factors by directly matching
their definition with the singular stresses. 

For convenience, the point on the boundary along the crack front $\theta=0$
(Figure ???) is considered. The distance from the crack tip to the
boundary is denoted as $L_{o}=r_{\eta}(\theta=0)$. The values of
the singular stresses at this point are equal to (Eq.~(\ref{eq:singularStress}))
\begin{equation}
\boldsymbol{\sigma}^{\mathrm{s}}(L_{o},\theta=0)=\sum_{i=I,II}c_{i}\boldsymbol{\psi}_{\sigma i}(\theta=0)\label{eq:singularStress_theta0}
\end{equation}
where $\boldsymbol{\psi}_{\sigma i}(\theta=0)$, the value of the
stress modes at $\theta=0$. It is obtained by interpolating $\boldsymbol{\psi}_{\sigma i}(\eta)$
at the discrete points of $\boldsymbol{\theta}(\eta)$. Alternatively,
the stresses at $\theta=0$, $\boldsymbol{\sigma}^{\mathrm{s}}(L_{o},\theta=0)$,
can be determined by interpolating the singular stresses $\boldsymbol{\sigma}^{\mathrm{s}}(L_{o},\eta)$
at discrete points.

Stress intensity factors can be computed directly from their definition
using the stresses in Eq.~(\ref{eq:singularStress_theta0}). For
a crack in a homogeneous medium, The classical definition of stress
intensity factors $K_{I}$ and $K_{II}$ for mode I and II are expressed
as 
\begin{equation}
\left\{ \begin{array}{c}
K_{I}\\
K_{II}
\end{array}\right\} =\sqrt{2\pi r}\left\{ \begin{array}{c}
\sigma_{\theta\theta}^{\mathrm{s}}(r,\theta=0)\\
\tau_{r\theta}^{\mathrm{s}}(r,\theta=0)
\end{array}\right\} \label{eq:GSIFdef-case1-2}
\end{equation}
Formulating Eq.~(\ref{eq:GSIFdef-case1-2}) at $r=L_{o}$ results
in
\begin{equation}
\left\{ \begin{array}{c}
K_{I}\\
K_{II}
\end{array}\right\} =\sqrt{2\pi L_{0}}\left\{ \begin{array}{c}
\sigma_{\theta\theta}^{\mathrm{s}}(L_{o},\theta=0)\\
\tau_{r\theta}^{\mathrm{s}}(L_{o},\theta=0)
\end{array}\right\} \label{eq:GSIFdef-case1-2-1}
\end{equation}
The stress intensity factors are then determined by substituting the
stress components $\sigma_{\theta\theta}^{\mathrm{s}}(L_{o},\theta=0)$
and $\tau_{r\theta}^{\mathrm{s}}(L_{o},\theta=0)$ obtained from Eq.~(\ref{eq:singularStress_theta0})
into Eq.~(\ref{eq:GSIFdef-case1-2-1}).

In the case of a crack at the interface between two isotropic materials,
the orders of singularity are a pair of complex conjugates $0.5\pm\mathrm{i}\epsilon$,
where the oscillatory index $\epsilon$ depends on the material properties.
The stress intensity factors are defined as:

\begin{equation}
\left\{ \begin{array}{c}
K_{I}\\
K_{II}
\end{array}\right\} =\sqrt{2\pi r}\left[\begin{array}{cc}
\cos(\epsilon\ln(r/L)) & \sin(\epsilon\ln(r/L))\\
-\sin(\epsilon\ln(r/L)) & \cos(\epsilon\ln(r/L))
\end{array}\right]\left\{ \begin{array}{c}
\sigma_{\theta\theta}^{\mathrm{(s)}}(r,0)\\
\tau_{r\theta}^{\mathrm{(s)}}(r,0)
\end{array}\right\} \label{eq:GSIFdef-case2-3}
\end{equation}
Formulating the definition (Eq.~(\ref{eq:GSIFdef-case2-3})) at $r=L_{o}$,
the stress intensity factors are expressed as
\begin{equation}
\left\{ \begin{array}{c}
K_{I}\\
K_{II}
\end{array}\right\} =\sqrt{2\pi L_{o}}\left[\begin{array}{cc}
\cos(\epsilon\ln(L_{o}/L)) & \sin(\epsilon\ln(L_{o}/L))\\
-\sin(\epsilon\ln(L_{o}/L)) & \cos(\epsilon\ln(L_{o}/L))
\end{array}\right]\left\{ \begin{array}{c}
\sigma_{\theta\theta}^{\mathrm{(s)}}(L_{o},0)\\
\tau_{r\theta}^{\mathrm{(s)}}(L_{o},0)
\end{array}\right\} \label{eq:GSIFdef-case2-3-1}
\end{equation}
where the singular stresses are obtained from Eq.~(\ref{eq:singularStress_theta0}). 

Although, it is out of the scope of this paper, it is worthwhile to
mention that the scaled boundary finite element method is capable
of modeling all types of stress singularity occurring at multi-material
junctions.

For a subdomain containing a crack tip, two of the eigenvalues are
equal to $1$. They represent the $T-$stress term and the rotational
rigid body motion term, which does not contribute to the stresses.
They are separated from other terms in Eq.~ (\ref{eq:singularStress_theta0})
and expressed as (superscript T for the $T-$stress) 
\begin{equation}
\boldsymbol{\sigma}^{T}(\eta)=\sum_{i=T_{I},T_{II}}c_{i}\boldsymbol{\psi}_{\sigma i}(\eta)\label{eq:TStress-1}
\end{equation}
The $T-$stress along the crack front ($\theta=0$) is determined
by interpolating the angular variation of the two stress modes $(\boldsymbol{\theta}(\eta),\boldsymbol{\psi}_{\sigma i}(\eta))$.
Alternatively, the interpolation can also be performed after obtaining
the angular variation of $\boldsymbol{\sigma}^{T}(\eta)$ from Eq.~(\ref{eq:TStress-1}).

Note that when evaluating the stress intensity factors or the $T-$stress,
only the corresponding modes are involved. It is not necessary to
evaluate the complete stress field. 
\end{document}

